Predicting Research Trends From Arxiv

We perform trend detection on two datasets of Arxiv papers, derived from its machine learning (cs.LG) and natural language processing (cs.CL) categories. Our approach is bottom-up: we first rank papers by their normalized citation counts, then group top-ranked papers into different categories based on the tasks that they pursue and the methods they use. We then analyze these resulting topics. We find that the dominating paradigm in cs.CL revolves around natural language generation problems and those in cs.LG revolve around reinforcement learning and adversarial principles. By extrapolation, we predict that these topics will remain lead problems/approaches in their fields in the short- and mid-term.

==> manual_analysis.tex <==
%\input{tables/topic_CL}
%\input{tables/topic_LG}

\section{Evaluation}
For both cs.CL and cs.LG, we identify the top-100 papers according to their z-score. We then (manually, initially) cluster these papers into groups in order to detect more general patterns: which areas will dominate in the upcoming years? In the following analysis, we focus on cs.LG, for space reasons. 
%In this section, we present the manual evaluation of top 100 papers from ``cs.CL'' and ``cs.LG''. %The evaluation  provides us with the ground-truth about the top trend in the corresponding research field, and enables further analysis. 

%\subsection{cs.CL}
%\input{plots/CL}
%We manually assign cs.CL papers into 13 categories, shown and %illustrated in Table \ref{table:topic_CL}. We mostly create %categories based on the NLP tasks around which the papers revolve. 
%%However, for papers that do not address specific NLP tasks, 
%We classify papers without a specific NLP task   according to other %criteria (described later). 

\input{plots/LG}
We assign cs.LG papers into 19 categories/topics.
%, listed and illustrated in Table \ref{table:topic_LG}. 
%\paragraph{Number of papers per category} %We first analyze the
We then introduce three statistical quantities to measure the importance of each category:
\begin{align*}
  n_C &= \sum_{p\in C} 1,\quad
  s_C = \sum_{p\in C} \text{z-score}(p),\quad
  m_C = \frac{1}{|C|}\sum_{p\in C} \text{z-score}(p).
\end{align*}
for each category $C=\{p_1,p_2,\ldots\}$ consisting of papers $p_1,p_2,\ldots$. The value $n_C$ gives the number of papers in each category. 
%\paragraph{Sum and mean of z-scores} We also calculated sum and mean z-scores for each category, shown in Figures \ref{fig:zscore_CL},  \ref{fig:zscore_mean_CL} and \ref{fig:zscore_sum_CL}. 
%The sum is the quantity:
%\begin{align*}
%  s_C = \sum_{p\in C} \text{z-score}(p)
%\end{align*}
%and the mean is the quantity:
%\begin{align*}
%  m_C = \frac{1}{|C|}\sum_{p\in C} \text{z-score}(p).
%\end{align*}
In contrast to $n_C$, the value $s_C$ does not only count the number of papers per category, but also weights them by their z-score. The value $s_C$ thus favors categories that have more top papers. The value $s_C$ favors categories whose average z-score is high; therefore, categories with very few papers may also rank highly. 

%The ranking based on $s_C$ is similar to that based on $n_c$, with a %few notable exceptions though. ``Model focused study [...]'' ranks %1st place according to $s_C$, while it only ranks 3rd place according %to $n_C$. ``adversarial example'' ranks 10th place according to $n_C$ %(containing only 3 papers), but 7th according to $s_C$. The ranking %based on $m_C$ highlights even more strongly that the 3 papers in the %category ``adversarial example'' rank very high in the list of top %100 papers because ``adversarial example'' ranks first according to %$m_C$, namely 2nd, 5th and 60th. \todo[inline]{SE: Fitz, please give %their exact ranks}\todo[inline]{Fitz: done}. In contrast, %``representation learning'' has one of the worst three $m_C$ values, %while having the largest $n_C$ value. We conjecture that these two %categories follow inverse trends: ``representation learning'' appears %to be declining, while ``adversarial example'' appears to be a rising %star.  
%different story; papers in smaller topics tend to have higher importance individually. Furthermore, three topics have significant higher z-scores: "Model focused study, not for specific NLP topic", "Adversarial example" and "Environment for artificial agent". High z-score of these topics probably come from different causes. Papers in "Model focused study...", on the one hand, are likely benefit from their wider audience group; i.e. studies on language model can be applies to various NLP tasks. On the other hand, "Adversarial example" is a new topic that addresses the issue that has significant real world implication.

%\subsection{cs.LG}
%Unlike cs.CL topics that base on long-term NLP tasks, cs.LG topics tend to be heavily influenced by the current popular machine learning model. 
\paragraph{Results} 
Given the current hype and success of deep learning, it is not surprising that most categories deal with different aspects of deep learning, see Fig.~\ref{fig:zscore_LG}. 
%Figures \ref{fig:num_LG},  \ref{fig:zscore_LG}, \ref{fig:zscore_mean_LG} and \ref{fig:zscore_sum_LG} %show the number of papers and z-score for each topic.
%rank papers based on $n_C$, $m_C$ and $s_C$. 
%\todo[inline]{SE: What's missing is description and illustration of categories like for cs.CL. In such tables, you should also list the titles of representative papers}
%\todo[inline]{Fitz: I don't know what kind of description/illustration to give cs.LG. For cs.CL, the description is to explain two non-NLP task based topics "model focused study..." and "extracting information...", and illustration is for "adversarial example". Because these three topics are likely unclear to readers even after going through cs.CL table. But for cs.LG, the information in the table cs.LG seems sufficient to me, and I don't know what other information to add.}
%\todo[inline]{Fitz: You want me to add "titles of representative papers" to cs.LG and cs.CL tables? Wouldn't it look too crowded? I tried to increase the table width, but the resulting table is not centered in the middle. Maybe you can set the right table width and I will add titles.}

The categories ``optimization [...]'', ``adversarial examples'' and ``reinforcement learning'' rank highest according to $n_C$ but the ranking is reversed according to $s_C$. As the biggest category, the majority of papers in ``optimization [...]'' focuses on the optimization process of deep learning models, like their saddle points, local minima, and properties of gradient descent. While optimization is a well-established field in machine learning, the fact that adversarial examples (how to attack deep learning models) and reinforcement learning rank higher according to $s_C$ may indicate that the field will be dominated more heavily by these two categories in the future. 
%``adversarial examples'' is a more important category in cs.LG than in cs.CL. 
%Interestingly, papers in this category mostly use image recognition as their testbed for new attack and defense method. The phenomenon could be a suggestion for upcoming popular research topic in cs.CL. 

``generative adversarial networks'' has rank 4 both according to $n_C$ and $s_C$. This area of machine learning deals both with \emph{generating data}, rather than classifying it as in traditional machine learning, and with fooling a machine learning system, as does ``adversarial examples'', but this time in order to render the system more robust. 
%Excluding categories with only 1 paper, ``reinforcement learning'', ``computer vision or nlp focused paper'' and ``generative adversarial example'' rank highest according to $m_C$. 
%Another noteworthy category is "searching NN [...]". Finding a good network structure has been a decisive factor for model performance in Deep Learning. A robust process can have many practical implications, e.g., good model performance, reducing computational and time costs in the finding process, and establishing a standard way to compare new model to the previous one. It is thus not surprising that many studies explore approaches that can automate the discovery of good network structure.
%``reinforcement learning'' and ``adversarial example'' have the highest z-score, and image recognition is the majority context for "adversarial example" research.

==> plots/LG.tex <==
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.8\textwidth]{plots/topic_num_LG.png}
%\caption{Topics and number of papers in it for cs.LG}
%\label{fig:num_LG} 
%\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{plots/zscore_LG.png}
\caption{Topics and corresponding z-score for cs.LG. Topics ranked by $n_C$ score. The score $s_C$ is on its original scale, and $m_C$ is multiplied with 10.}
\label{fig:zscore_LG} 
\end{figure}

%\begin{figure}[h]
%\centering
%\includegraphics[width=0.8\textwidth]{plots/topic_zscore_mean_LG.png}
%\caption{Topics and corresponding z-score(mean) for cs.LG}
%\label{fig:zscore_mean_LG} 
%\end{figure}

%\begin{figure}[h]
%\centering
%\includegraphics[width=0.8\textwidth]{plots/topic_zscore_sum_LG.png}
%\caption{Topics and corresponding z-score(sum) for cs.LG}
%\label{fig:zscore_sum_LG} 
%\end{figure}
